Maximum Bayes Smatch Ensemble Distillation for AMR Parsing

AMR parsing has experienced an unprecendented increase in performance in the last three years, due to a mixture of effects including architecture improvements and transfer learning. Self-learning techniques have also played a role in pushing performance forward. However, for most recent high performant parsers, the effect of self-learning and silver data augmentation seems to be fading. In this paper we propose to overcome this diminishing returns of silver data by combining Smatch-based ensembling techniques with ensemble distillation. In an extensive experimental setup, we push single model English parser performance to a new state-of-the-art, 85.9 (AMR2.0) and 84.3 (AMR3.0), and return to substantial gains from silver data augmentation. We also attain a new state-of-the-art for cross-lingual AMR parsing for Chinese, German, Italian and Spanish. Finally we explore the impact of the proposed technique on domain adaptation, and show that it can produce gains rivaling those of human annotated data for QALD-9 and achieve a new state-of-the-art for BioAMR.

==> figure2.tex <==

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{AAAI2022_amrbasic.png}
%     \caption{AMR graph for \textit{The girls repaired the machines}. The nodes represent the concepts \textit{girl, machine, repair-01} and the edges correspond to the roles \textit{:ARG0, :ARG1}. Dotted lines indicate implicit alignments between the input tokens and the AMR concepts.}
%     \label{fig:AAAI2022_amrbasic}
% \end{figure}


\begin{figure}
    \centering

\begin{tikzpicture}

\node (w0) at (0.0,0) {The};
\node [right = 10pt of w0] (w1) {\strut students};
\node [right = 10pt of w1] (w2) {\strut repaired};
\node [right = 10pt of w2] (w3) {\strut the};
\node [right = 10pt of w3] (w4) {\strut machines};

\node [draw,rounded corners,fill={rgb:white,15;green,1;blue,1}, above = 80pt of w2] (0) {repair-01};
\node [draw,rounded corners,fill={rgb:white,15;green,1;blue,1},
above = 20pt of w1] (0_0) {student};
\node [draw,rounded corners,fill={rgb:white,15;green,1;blue,1},
above = 20pt of w4] (0_1) {machine};
\draw [-latex,thick] (0) -- node[left,pos=0.5]  {\footnotesize :ARG0} (0_0);
\draw [-latex,thick] (0) -- node[right,pos=0.5]  {\footnotesize :ARG1} (0_1);

\draw [dashed] (0_0) -- (w1);
\draw [dashed] (0_1) -- (w4);
\draw [dashed] (0) -- (w2);

\end{tikzpicture}

    \caption{AMR graph for \textit{The students repaired the machines}. The nodes represent the concepts \textit{student, machine, repair-01} and the edges correspond to the roles :ARG0, :ARG1. Dotted lines indicate implicit alignments between the input tokens and the AMR concepts.}
    \label{fig:AAAI2022_amrbasic}
\end{figure}

==> limitation.tex <==
\section{Limitations}

Smatch has its own issues: Re-entrancies are not scored properly
Decoding speed of joint-voc with silver data
